Power Line Inspection Tasks with Multi-Aerial Robot Systems via Signal Temporal Logic Specifications

A framework for computing feasible and constrained trajectories for a fleet of quad-rotors leveraging on Signal Temporal Logic (STL) specifications for power line inspection tasks is proposed in this paper. The planner allows the formulation of complex missions that avoid obstacles and maintain a safe distance between drones while performing the planned mission. An optimization problem is set to generate optimal strategies that satisfy these specifications and also take vehicle constraints into account. Further, an event-triggered replanner is proposed to reply to unforeseen events and external disturbances. An energy minimization term is also considered to implicitly save quad-rotors battery life while carrying out the mission. Numerical simulations in MATLAB and experimental results show the validity and the effectiveness of the proposed approach, and demonstrate its applicability in real-world scenarios.

==> figure/pipeline_diagram.tex <==
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\tikzset{
  state/.style={
    rectangle,
    draw=black, very thick,
    minimum height=1.0em,
    text centered,
  },
}

\begin{tikzpicture}[->,node distance=3.0cm,scale=1.0, every node/.style={scale=1.0}]

  %%{ nodes

  \node[state, shift = {(0.0, 0.0)}] (navigation) {
      \begin{tabular}{c}
        \footnotesize Motion\\
        \footnotesize Planner
      \end{tabular}
    };

  \node[state, right of = navigation, shift = {(-0.3, 0)}] (controller) {
      \begin{tabular}{c}
        \footnotesize Reference \\
        \footnotesize controller
      \end{tabular}
    };

  \node[state, right of = controller, shift = {(0.1, -0)}] (attitude) {
      \begin{tabular}{c}
        \footnotesize Rate\\
        \footnotesize controller
      \end{tabular}
    };

  \node[state, right of = attitude, shift = {(0.2, -0)}] (actuators) {
      \begin{tabular}{c}
        \footnotesize Actuators
      \end{tabular}
    };

  \node[state, below of = actuators, shift = {(0.0, 2.25)}] (sensors) {
      \begin{tabular}{c}
        \footnotesize Sensors
      \end{tabular}
    };

  \node[state, below of = attitude, shift = {(0, 1.2)}] (estimator) {
      \begin{tabular}{c}
        \footnotesize State \\
        \footnotesize estimator
      \end{tabular}
    };

  \node[state, right of = estimator, shift = {(-0.6, 0.0)}] (localization) {
      \begin{tabular}{c}
        \footnotesize Localization
      \end{tabular}
    };

  %%}

  %%{ paths

  \path[->] ($(navigation.east) + (0.0, 0)$) edge [] node[midway, shift = {(0.0, 0.0)}] {
      \begin{tabular}{c}
        \footnotesize $\mathbf{x^\star}, \mathbf{u^\star}$\\
        \footnotesize $\psi$
    \end{tabular}} ($(controller.west) + (0.0, 0.00)$);

  \path[->] ($(controller.east) + (0.0, 0)$) edge [] node[midway, shift = {(0.0, 0.0)}] {
      \begin{tabular}{c}
        \footnotesize $\bm{\omega}_d$, $T_d$\\
        \footnotesize \SI{100}{\hertz}
    \end{tabular}} ($(attitude.west) + (0.0, 0.00)$);

  \path[->] ($(attitude.east) + (0.0, 0)$) edge [] node[midway, shift = {(0.0, 0.0)}] {
      \begin{tabular}{c}
        \footnotesize $\bm{\tau}_d$ \\
        \footnotesize $\approx$\SI{1}{\kilo\hertz}
    \end{tabular}} ($(actuators.west) + (0.0, 0.00)$);

  \path[-] ($(estimator.west)+(0, 0)$) edge [] node[above, midway, shift = {(-1.8, -0.1)}] {
      \begin{tabular}{c}
        \footnotesize $\mathbf{\zeta}$, $\mathbf{R}$, $\bm{\omega}$\\
        \footnotesize \SI{100}{\hertz}
    \end{tabular}} ($(controller.south |- estimator.west)$) -- ($(controller.south |- estimator.west)$) edge [->,] ($(controller.south)+(0, 0)$);

  \path[->] ($(controller.south |- estimator.west)+(0, 0)$) edge [] ($(controller.south)$);

  \draw[-] ($(attitude.south) + (0.0, -0.15)$) edge [->] node[right, midway, shift = {(-0.2, 0.0)}] {
      \begin{tabular}{c}
        \footnotesize $\mathbf{R}$, $\bm{\omega}$
    \end{tabular}} ($(estimator.north) + (0.0, 0.0)$);

  \draw[-] ($(sensors.south)+(0.4, 0)$) -- ($(sensors.south |- localization.east) + (0.4, 0)$) edge [->] ($(localization.east)$);

  \draw[->] ($(localization.west)+(0, 0)$) -- ($(estimator.east)$);

  %%}

  %%{ backgrounds

  \begin{pgfonlayer}{background}
    \path (actuators.west |- actuators.north)+(-0.15,0.47) node (a) {};
    \path (sensors.south -| actuators.east)+(+0.15,-0.15) node (b) {};
    \path[fill=gray!3,rounded corners, draw=black!70, densely dotted]
      (a) rectangle (b);
  \end{pgfonlayer}
  \node [rectangle, above of=actuators, shift={(0.0,0.00)}, node distance=1.7em] (autopilot) {\footnotesize UAV plant};

  \begin{pgfonlayer}{background}
    \path (attitude.west |- attitude.north)+(-0.15,0.47) node (a) {};
    \path (attitude.south -| attitude.east)+(+0.15,-0.15) node (b) {};
    \path[fill=gray!3,rounded corners, draw=black!70, densely dotted]
      (a) rectangle (b);
  \end{pgfonlayer}
  \node [rectangle, above of=attitude, shift={(0,0.2)}, node distance=1.7em] (autopilot) {\footnotesize Autopilot};

  %%}

\end{tikzpicture}

